BT-ACTION: A Test-Driven Approach for Modular Understanding of User Instruction Leveraging Behaviour Trees and LLMs

Natural language instructions are often abstract and complex, requiring robots to execute multiple subtasks even for seemingly simple queries. For example, when a user asks a robot to prepare avocado toast, the task involves several sequential steps. Moreover, such instructions can be ambiguous or infeasible for the robot or may exceed the robot's existing knowledge. While Large Language Models (LLMs) offer strong language reasoning capabilities to handle these challenges, effectively integrating them into robotic systems remains a key challenge. To address this, we propose BT-ACTION, a test-driven approach that combines the modular structure of Behavior Trees (BT) with LLMs to generate coherent sequences of robot actions for following complex user instructions, specifically in the context of preparing recipes in a kitchen-assistance setting. We evaluated BT-ACTION in a comprehensive user study with 45 participants, comparing its performance to direct LLM prompting. Results demonstrate that the modular design of BT-ACTION helped the robot make fewer mistakes and increased user trust, and participants showed a significant preference for the robot leveraging BT-ACTION. The code is publicly available at https://github.com/1Eggbert7/BT_LLM.

==> sections/03_1method_Olek.tex <==
\section{Methodology: \frameworkName}

\label{ch:methodology}

%In this section, we describe the \frameworkName framework, how it works, how it is constructed, and how it compares to the baseline system, with a brief introduction of the baseline system.

\subsection{Overview}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{img/Example Seq.png}
    \caption{An example set of actions for task \( T_i\) (preparing bacon and egg sandwich), each composed of step-by-step high-level robot actions, \( T_i = \{a_0,...,a_8\}\),  \(a_j \in A \)}
    \label{fig:Seq-example}
\end{figure}

Given a user instruction \( u \), the goal of \frameworkName is to generate a set of robot actions that would fulfill the task specified in \( u \).
Accordingly, each task \( T_i \) is composed of a set of \(a_j \in A\) that should be executed step by step, \( T_i~=~\{a_0 \dots a_j\} \) (see Figure~\ref{fig:Seq-example}). Moreover, \(\mathcal{T}~=~\{T_0 \dots T_n\} \) shows the set of tasks that the robot is familiar with.
%%%%%%%Alex version here
%Given a user instruction \( u \), the goal of \frameworkName is to determine which known action \(T_i \in \mathcal{T} = \{T_0, T_1, ..., T_n\} \) fulfills the instruction. %If no existing sequence is suitable, the system generates a new sequence \( a_{n+1} \) using the LLM. 
%Each task \( T_i \) consists of high-level robot actions form the set  \(A =\{a_0,a_1,...,a_k\}\) that should be executed step by step to complete the task (see Figure~\ref{fig:Seq-example}).


To comprehend and act upon the user instructions, \frameworkName suggests four main functions that the constructed behavior tree handles: Classification, Information, Sequence generation, and Error Handling. Classification enables more fine-tuned handling of user instructions through LLM-based condition nodes; information ensures explanations and transparency in robot behavior; sequence generation creates new action plans when required; and error handling solidifies the robustness of the framework by checking for potential mistakes.
%First, to classify a user request, the framework uses condition nodes in the BT to categorize the user request. Once \frameworkName classifies the user input into one of the categories (either ambiguous, clear, modification, or infeasible), it triggers a corresponding subtree responsible for providing information that communicates to an LLM. %the conversation history with the classification to generate a response with a clarification request or answer. The robot clarifies back to the user what it understood. 
%For example, if the user ambiguously asked for \textit{``something sweet''}, then this request should be classified as ambiguous, and the robot could respond with \textit{``There are multiple options that fit your request. Would you like some pancakes with maple syrup and berries or perhaps a peanut butter and jelly sandwich?''}. 
%If the request is classified as a modification, the sequence generation is triggered to prompt the LLM to synthesize new task actions in JSON format tailored to the user’s instruction.
%\frameworkName also includes error-handling mechanisms implemented through action and condition nodes. For example, if a user request is mapped to a task that the robot could execute, an action node called \texttt{CheckMapping} is triggered to ensure the mapping is correct, and a condition node checks if the user request maps to only one possible task.
A simplified version of the \frameworkName can be seen in Figure~\ref{fig:simplified_tree}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/Simplified Tree.png}
    \caption{Simplified Behavior Tree of the \frameworkName System.}
    \label{fig:simplified_tree}
\end{figure*}

\subsubsection{Classification}

\frameworkName leverages the modular structure of BTs to systematically process and classify user instructions $u$ into the following categories:



\[\footnotesize
C(u) =
\begin{cases} 
\text{Ambiguous}, & \text{if clarification is required,} \\
\text{Clear}, & \text{if it directly maps to a known sequence,} \\
\text{Modification}, & \text{if modification of a known task is needed,} \\
\text{Infeasible}, & \text{if beyond the robots capabilities.}
\end{cases}
\]

%The classification is implemented through a series of condition nodes in the behavior tree. Each condition node invokes a tailored LLM prompt to check whether the user input fits a particular category—starting with ambiguity detection, followed by checks for known task matches and feasibility. 

This classification is implemented through a sequence of condition nodes in the behavior tree, each using a tailored LLM pre-prompt, for example: \textit{``Based on the user instruction and history, is the request ambiguous?''} or \textit{``Does the instruction match a known task''}. This classification starts with ambiguity detection and is followed by checks for known task matches and feasibility. Concretely, classification proceeds through a stepwise series of binary checks:
\begin{equation}
   C(u) = \texttt{LLM}(f(u) \oplus g(H)),
\end{equation}
%\[
%\begin{aligned}
%\text{IsAmbiguous}(x) &= %\text{LLM}_1(f(x) \oplus g(H)) \\
%\text{IsClear}(x) &= \text{LLM}_2(f(x) \oplus g(H)) \\
%\text{IsModification}(x) &= \text{LLM}_3(f(x) \oplus g(H)) \\
%\text{IsInfeasible}(x) &= \text{LLM}_4(f(x) \oplus g(H)) \\
%\end{aligned}
%\]
where \( f(u) \) embeds the user instruction into prompt-ready format, and \( g(H) \) encodes the current conversation history. Each check corresponds to a condition node in the behavior tree, and the first one returning true determines the classification and activates the corresponding subtree.


\begin{comment}
The categories are specifically defined as follows:
    


\textbf{(a) Clear Instructions:}
If the request directly matches a predefined sequence, it is classified as clear, and nodes for execution of the sequence are triggered.

\textbf{(b) Ambiguous Instructions:}
If the request lacks specificity or invites multiple possible interpretations, it is classified as ambiguous, and the robot asks follow-up questions using clarification nodes.

\textbf{(c) Modification Instructions:}
If the request requires \textbf{modification} to a known task (e.g., "Make pancakes but add double syrup"), it is considered to require a new sequence, triggering further nodes for sequence generation.

\textbf{(d) Infeasible Instructions:}
If the request involves an action beyond the robot's capabilities (e.g., "Repaint the kitchen walls"), it is classified as \textbf{infeasible}, and action nodes for structured rejection responses are triggered.

\end{comment}



\subsubsection{Information} \label{sec:clarifciation}
\label{sec:information}
After classification, the robot’s goal is to communicate its intended actions back to the user based on the classification category: %Based on the classification the clarification is structured as such:


(a) If \( C(u) = \texttt{Clear} \), the framework identifies a matching known task \(T_i \in \mathcal{T}, i \in \{1,...,n\} \) from the set of known tasks. This match is verified through internal error-handling nodes (such as \texttt{CheckMapping} and \texttt{KNOWNO}). Once validated, the LLM is prompted to provide the known task name of $T_i$ for acknowledging users about the execution, $\texttt{LLM}(T_i)$, such as \textit{``I'll get started on the task for a bacon and egg sandwich''}.


(b) If \( C(u) = \texttt{Ambiguous} \), the LLM is prompted to generate a follow-up question: \(
Q \leftarrow \texttt{LLM}(g(H), \mathcal{T}, P_{\text{follow-up}}),
\)
where \( g(H) \) encodes the full conversation history, \( \mathcal{T} = \{T_0, T_1, ..., T_n\} \) is the set of known tasks, and \( P_{\text{follow-up}} \) is a structured pre-prompt instructing the LLM to suggest similar tasks based on the conversation history and to inquire if the user has something else in mind.
\frameworkName then outputs possible matching options, e.g., \textit{``There are multiple options that might fit your request. Would you like some pancakes with maple syrup and berries or perhaps a peanut butter and jelly sandwich?''}. The user's reply \( r \) is appended to the conversation history \( H \leftarrow H \cup \{(Q, r)\} \), and the behavior tree is re-triggered from the root with the updated context.


(c) If \( C(u) = \texttt{Modification} \), the system triggers the sequence generation process (see Section~\ref{sec:seqgen}) to generate a new task \( T_{n+1} \). Then, LLM is prompted to summarize \( T_{n+1} \) for user confirmation, $\texttt{LLM}(T_{n+1})$, such as \textit{``To fulfill your request, I will fry two pieces of bacon and an egg, then put it on a toast and serve. Does this sound good to you?''}. If the user confirms, the sequence is accepted as the result of the interaction with the user; if not, a fallback is triggered to ask users to restate their instruction in a clearer way.
%if not, a fallback clarification is triggered, that prompts the user to restate the instruction in a clearer way.

(d) If \( C(u) = \texttt{Infeasible} \), the robot informs the user that their request cannot be fulfilled due to resource or constraint limitations. %This classification can result from multiple condition nodes, such as an LLM-based capability check (e.g., unsupported actions like \textit{“repaint the kitchen walls”}) or a feasibility check verifying available ingredients and realistic quantities (e.g., requests for \textit{``oyster mushrooms''} or \textit{``100 eggs''}).
Depending on which condition node triggered the classification, the robot communicates an appropriate explanation using the LLM:
\(
y \leftarrow \texttt{LLM}(u, A, I, P_{\text{explanation}})
\)
where
%- \( u \) is the original user instruction,
%- \( A \) is the set of high-level robot functions,
\( I \) is the set of existing ingredients, and \( P_{\text{explanation}} \) is a structured prompt guiding the LLM to explain why the task is infeasible. Example responses might include: \textit{``I’m sorry, but I cannot repaint the kitchen walls as I lack the necessary tools.''}
or
\textit{``I cannot make this request as it includes ‘goat cheese’, which is not part of my known ingredients.''}
The user’s response \( r \) is appended to the conversation history:
\(
H \leftarrow H \cup \{(u, r)\}
\),
and the behavior tree is re-triggered from the root with the updated context.


\subsubsection{Sequence generation}
\label{sec:seqgen}
When a user instruction is classified as a modification, the system prompts the LLM to generate a new task action set $T_{n+1}$: %This plan is based on the conversation history and the original known sequence, and it outlines the steps the robot should take to fulfill the modification request. %This process is captured by the following formulation:
%Specifically, for the given user instruction \( u \) and the current conversation history \( H \), if the instruction is classified as a modification, the LLM is prompted as follows:
%\[
\begin{equation}
T_{t+1} \leftarrow \texttt{LLM} (f(u) \oplus g(H) \oplus w(\mathcal{T})),
\end{equation}
%\]
where \( f(u) \) embeds the instruction into prompt-ready format, \( g(H) \) encodes the full conversation history, and \( w(\mathcal{T}) \) lists all known tasks \( \{T_0,\dots, T_n\} \).
%Then, the LLM generates a new sequence:
%\[
%\begin{equation}
%a_{n+1} \leftarrow \text{LLM}(p),
%\end{equation}
%\]
The output \( T_{n+1} \) is the set of robot action functions to fulfill the query $u$. An example output of such a generated sequence can be seen in Figure~\ref{fig:Seq-example}.




\subsubsection{Error Handling}


%In addition to classification of the user input, 
The framework also incorporates the following error-handling to further support robustness and avoid LLM hallucinations (see Table~\ref{tab:error-nodes}).


(a) \texttt{KNOWNO:} 
 This safety check is integrated after the initial classification, particularly in cases labeled as \texttt{Clear}, to verify whether the user instruction maps to only one known task.
%Another error-handling mechanism used in \frameworkName is 
KNOWNO is a framework that measures the uncertainty of LLM-based planners~\cite{ren_robots_2023}. 
It takes the user request \( u \) as input and returns a set of tasks \( T = \{T_0,\dots, T_n\} \) that potentially fulfill the request. If multiple mappings are found, a clarification node is triggered to disambiguate the user's intent.

(b) \texttt{CheckMapping:}
Used when the KNOWNO framework returns a single matching task \( T_i \). This node prompts the LLM with the user instruction \( u \), history \( H \), and \( T_i \), asking whether the task aligns with the user’s intent. If uncertain, further nodes to check for modification are triggered.


(c) \texttt{CheckNewSeq:}
In the case of a modification request, the LLM-generated sequence $T_{n+1}$ is passed through error-handling nodes for validation,
\(
%\text{isValid}(T_{n+1}) %\leftarrow
\texttt{CheckNewSeq}(T_{n+1})
\).
The \texttt{CheckNewSeq} is a custom node to ensure all actions are part of the predefined set of valid robot actions \( A = \{a_0,\dots, a_n\} \), and all mentioned ingredients exist within the existing ingredient list \( I = \{i_0,\dots, i_m\} \) to avoid LLM hallucinations.


%If valid, the robot clarifies the generated sequence with the user before execution. If invalid, a fallback clarification node is triggered to ask for user clarification or reject the request. The error-handling nodes can be seen in Table~\ref{tab:error-nodes}.

\begin{comment}
The \texttt{CheckNewSeq} node is a custom Python function that performs a structured validation of the LLM-generated JSON sequence. It checks whether:
\begin{enumerate}[label = (\roman*)]
    \item the sequence is syntactically valid JSON, 
    \item all actions are part of the predefined set of valid robot actions \( A = \{a_0,\dots, a_n\} \), 
    \item the parameters match expected types (e.g., numeric values or valid ingredient names), and 
    \item all mentioned ingredients exist within a predefined ingredient list \( I = \{i_0,\dots, i_m\} \). 
\end{enumerate}
These checks involve parsing the function signatures and validating types and content based on structured JSON definitions.

If valid, the robot clarifies the generated sequence with the user before execution. If invalid, a fallback clarification node is triggered to ask for user clarification or reject the request. The error-handling nodes can be seen in Table~\ref{tab:error-nodes}.
\end{comment}

\begin{table}[t]
    \centering
    \caption{Error-handling nodes}
    \begin{tabular}{ll}
         \textbf{Error-Handling Node} & \textbf{Function} \\
         \hline
         \hline
        \verb|KNOW NO|~\cite{ren_robots_2023} & Ensures correct mapping of user instruction\\
        \hline
        \verb|CheckMapping| & Validates task-action alignment\\
        \hline
        \verb|RunSafetyCheck| & Filters infeasible requests (e.g., 500 eggs).\\
        \hline
        \verb|CheckNewSeq| & Ensures syntax and resource validity.\\
    \end{tabular}
    \label{tab:error-nodes}
\end{table}



(d) \texttt{RunSafetyCheck:}
Triggered after a \texttt{Modification} classification, this node uses an LLM prompt to assess whether the request is feasible in terms of available ingredients and reasonable quantities. The prompt encodes the ingredient set \( I = \{i_0,\dots,i_m\} \) and defines acceptable quantity limits (e.g., under 10 units). If constraints are violated, the node triggers fallback clarification.

Note that \texttt{RunSafetyCheck} also functions as a classification node in cases where the instruction is deemed infeasible. If ingredient constraints or quantity limits are violated, the task is classified as \texttt{Infeasible}, and a response is generated accordingly (see Section~\ref{sec:information}


%Original version if we want to go back
\begin{comment}

(b) \texttt{KNOWNO:} Another error-handling mechanism used in \frameworkName is the KNOWNO framework, "a framework for measuring and aligning the uncertainty of LLM-based planners such that they \textit{know when they don’t know} and ask for help when needed"~\cite{ren_robots_2023}. KNOWNO is integrated as an action node after the initial classification, particularly in cases labeled as clear, to verify whether the user instruction maps confidently to only one known task. It takes the user request \( u \) as input and returns a set of tasks \( T = \{T_0,\dots, T_n\} \) that potentially fulfill the request. If multiple mappings are found, a clarification node is triggered to disambiguate the user's intent.
    
\end{comment}

\subsubsection{Execution Flow Overview}
An overview of how a user instruction is processed through the behavior tree is shown in Algorithm~\ref{alg:btplan}. This algorithm reflects the modular nature of \frameworkName and its ability to flexibly route requests through classification, sequence generation, clarification, and execution.


\begin{algorithm}[t!]
\caption{Behavior Tree Processing Logic in \frameworkName}
\label{alg:btplan}
\begin{algorithmic}[1]
\State $u \leftarrow$ User instruction
\State $H \leftarrow$ Conversation history
\State $C(u) \leftarrow$ Classify input as \texttt{Ambiguous}, \texttt{Clear}, \texttt{Modification}, or \texttt{Infeasible}
\If{$C(u) = \texttt{Clear}$}
    \State Trigger known sequence execution
\ElsIf{$C(u) = \texttt{Ambiguous}$}
    \State Trigger clarification node with multiple options
\ElsIf{$C(u) = \texttt{Modification}$}
    \State Construct prompt $p \leftarrow f(u) \oplus g(H) \oplus w(T)$
    \State $T_{n+1} \leftarrow \texttt{LLM}(p)$
    \State \texttt{CheckNewSeq}($T_{n+1}$)
    \If{valid}
        \State Clarify $T_{n+1}$ with user
        \If{confirmed}
            \State Execute $T_{n+1}$, acknowledge users
        \Else
            \State Ask for further clarification
        \EndIf
    \Else
        \State Trigger fallback clarification node
    \EndIf
\ElsIf{$C(u) = \texttt{Infeasible}$}
    \State Inform user about infeasibility
\EndIf
\end{algorithmic}
\end{algorithm}


\subsection{LLM Prompt Integration}
The pre-prompts in \frameworkName are tailored for specific actions or decision points. Each action and condition node dynamically integrates the full conversation history between the user and the robot, allowing the LLM to generate contextually relevant responses by considering prior interactions and clarifying ambiguities.

\subsection{Implementation Details}
\label{sec:softwareDevelopment}

The \frameworkName Framework was implemented in Python, using \texttt{PyTrees} to construct and manage the behavior tree and the OpenAI API ChatGPT 4o-mini model for natural language processing. The modular design allowed each node—e.g., ambiguity classification or feasibility checking—to be developed and tested independently before integration.

This structure enabled incremental debugging and ensured that system behavior remained explainable and predictable. Each node incorporated tailored prompts, dynamically including the user’s instruction and conversation history. By classifying user inputs within the BT, the framework provided targeted feedback—for example, routing infeasible requests to a rejection node that responds with messages like, \textit{``Sorry, but this is outside my capabilities''}.

Such modularity enhanced transparency and user understanding, reinforcing the framework’s goal of structured and context-aware interaction in HRI settings.

\subsection{Baseline System}
The baseline system served as a comparison for evaluating the performance of \frameworkName. It relied on a single pre-prompt loaded into the ChatGPT-4o-mini API to handle all user instructions and generate responses. The prompt encoded the system's capabilities, known sequences, ingredients, and functions. See Section \ref{sec:preevaluation} for details on how we developed the prompt. 

==> sections/03_method.tex <==
\section{Methodology: BT and LLM Framework}

\label{ch:methodology}

This chapter describes the development and structure of the proposed system.% used in the experiment, including the Baseline System and the BT-LLM Framework. 
It covers the system architecture, software development, and implementation details.

\subsection{Overview of the Framework}

The BT-LLM Framework processes user inputs through a modular decision-making structure, leveraging behavior trees to ensure systematic and explainable task handling. Key features like \textbf{ambiguity management}, \textbf{error handling}, and \textbf{structured sequence generation} enhance the system's reliability and user instruction comprehension.

The BT-LLM Framework processes user instructions through a structured sequence of decision-making steps. These include ambiguity classification, verification against predefined sequences, feasibility checks, and sequence generation when needed. %A detailed breakdown of these steps, along with illustrative examples, is provided in Section~\ref{sec:Case-Study}. Figure~\ref{fig:simplified_fsm} illustrates the decision-making process in the form of a flow diagram. 
This structured approach ensures that all user requests are either mapped to known actions, clarified, or evaluated for feasibility before execution. Figure~\ref{fig:simplified_tree} shows this process in the form of a simplified Behavior Tree and Figure~\ref{fig:full_bt_architecture} shows the full Behavior Tree that was used to implement the framework.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textheight]{img/Simplified FSM of Tree.png}
    \caption{Finite-State Machine Representation of the Simplified Behavior Tree.}
    \label{fig:simplified_fsm}
\end{figure*}


\subsection{Case Study}
\label{sec:Case-Study}

This case study illustrates the application of the BT-LLM framework in a home kitchen assistant scenario, providing a concrete example to clarify abstract concepts and evaluate its effectiveness in this specific context. While the framework's structure suggests potential adaptability to other domains, this study does not test its application beyond the kitchen assistant setting.

Furhat, a socially interactive robot, was set up as a kitchen assistant capable of theoretically managing other kitchen robots and aiding users with tasks like meal preparation or cleaning. Users interacted with Furhat through natural language, issuing instructions or asking questions such as \textit{\textquotedblleft Can you make me a sandwich?\textquotedblright}, \textit{\textquotedblleft What sweet breakfast options can you make me?\textquotedblright}, or \textit{\textquotedblleft Can you repaint the kitchen walls?\textquotedblright}.

The system processed these requests by classifying them based on the structured approach described in Section~\ref{sec:BT-Node-Implementation}. Depending on whether a request was \textbf{ambiguous, a known task, a feasible but new sequence, or infeasible}, Furhat either responded immediately, sought clarification, or adapted existing sequences accordingly.

For example, if a user requested \textbf{a predefined task}, such as \textit{"Make me a bacon and egg sandwich"}, the system classified it as a request for a known sequence and directly mapped it to an existing execution sequence (see Figure~\ref{fig:Seq-example}). If a user request \textbf{required modifications}, such as \textit{"Make me pancakes but double the syrup and no berries"}, the system classified the request as \textbf{new sequence} and adjusted the relevant sequence before execution.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{img/Example Seq.png}
    \caption{An example of a JSON high-level sequence to generate a bacon and egg sandwich.}
    \label{fig:Seq-example}
\end{figure}

Although centered on a kitchen assistant, the BT-LLM framework was designed for broader applications. For instance, a museum guide robot could use the framework to answer visitor questions about exhibits, provide tailored recommendations, or explain its limitations in handling certain queries. Similarly, in industry, a warehouse robot could manage inventory, generate sorting sequences, or reject infeasible actions. By leveraging behavior trees, the framework ensured modularity, transparency, and adaptability across diverse robotic applications involving natural language interactions.


\subsection{Research Process} \label{sec:researchProcess}

The research process outlined in Figure~\ref{sec:researchProcess} involved identifying the challenges of enhancing LLM reliability and explainability in HRI, followed by developing a BT-LLM framework. A baseline system relying on a single pre-prompt was implemented for comparison prior to the development of the framework. Testing and debugging ensured consistent behavior. User experiments were planned to evaluate task error rates, trust, and user comfort using metrics such as RoSAS and MDMT. The data from the experiments was analyzed statistically to compare the performance of the two systems.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{img/Research Process.png}
    \caption{Research process overview.}
    \label{fig:research-process}
\end{figure}


\section{BT-LLM Framework}
The BT-LLM Framework improved upon the baseline system by structuring tasks into modular decision nodes within a behavior tree. This approach worked well before for research in HRI~\cite{elkady_structured_2013, moubarak_modular_2012, dorigo_behavior_2018}. It allowed for fine control of task flow and ensured that user interactions were handled in a systematic and predictable manner. Features like \textbf{error handling}, \textbf{ambiguity management}, and \textbf{structured sequence generation} enhanced the system’s reliability and user instruction comprehension. The integration of BT with the LLM introduced a logical and modular way to manage user inputs and produce reliable responses.






\subsection{BT Node Implementation in the Framework}
\label{sec:BT-Node-Implementation}

The BT-LLM Framework builds on the general principles of behavior trees but integrates decision-making nodes tailored for human-robot interaction. This section details how BT nodes were specifically adapted to process user instructions.

\paragraph*{LLM-Based Action Nodes}
Action nodes trigger direct interactions with the LLM to handle ambiguity, generate responses, or execute predefined robotic actions. Given a user request \( x \), an action node formulates a structured response:

\[
A(x, h) = f(x, h)
\]

where \( x \) represents the user-requested sequence, \( h \) denotes the conversation history, and \( f(x, h) \) is a function that constructs the system response. This approach ensures clarity by explicitly stating the action being performed while maintaining context from prior interactions.

For example, an action node for ambiguity resolution takes the conversation history and generates a clarification prompt as seen in Figure~\ref{alg:printAmbiguousAnswer}.

\begin{figure}[ht]
\centering
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State \textbf{class} \textsc{PrintAmbiguousAnswer} \textbf{inherits from} \textsc{Behaviour}
\Function{Update}{}
    \If{LLM is available}
        \State Generate ambiguous response using LLM and conversation history
        \State Append the response to the conversation history
        \State \Return Success
    \Else
        \State \Return Failure
    \EndIf
\EndFunction
\end{algorithmic}
\end{algorithm}
\caption{Action Node pseudocode for ambiguous input handling.}
\label{alg:printAmbiguousAnswer}
\end{figure}

A simplified example of this ambiguity-handling process is shown in Figure~\ref{fig:bt-ambiguous-example}.

\paragraph*{Classification with Condition Nodes}
Condition nodes in the BT-LLM Framework enable structured classification of user instructions before executing an action. These nodes act as decision points that determine how an instruction should be processed by querying the LLM and categorizing input accordingly.

Each condition node evaluates a user instruction \( x \) and classifies it into a specific category. The framework utilizes multiple condition nodes to refine this classification progressively:

\[\footnotesize
C(x) =
\begin{cases} 
\text{Ambiguous}, & \text{if clarification is required} \\
\text{Clear}, & \text{if it directly maps to a known sequence} \\
\text{New Sequence}, & \text{if modification of a known task is needed} \\
\text{Infeasible}, & \text{if beyond system capabilities}
\end{cases}
\]

\paragraph*{Ambiguity Classification}
One of the first condition nodes determines whether a request is ambiguous, meaning it lacks specificity or invites multiple possible interpretations. If classified as ambiguous, the framework triggers an action node with a \textbf{LLM clarification prompt} before proceeding further. This classification step is implemented using an LLM-based condition node, the prompt for it can be seen in Figue~\ref{fig:pre-prompt-ambiguous}.

\paragraph*{Further Classification and Task Execution}
If a request is not ambiguous, it is further classified by additional condition nodes:
\begin{itemize}
    \item \textbf{Known Sequences:} If the request directly matches a predefined sequence, it is classified as \textbf{clear} and nodes for execution of the sequence are triggered.
    \item \textbf{New Sequence Generation:} If the request requires modifications to a known task (e.g., "Make pancakes but add double syrup"), it is classified as a \textbf{new sequence}, triggering further nodes for sequence generation.
    \item \textbf{Feasibility Check:} If the request involves an action beyond the robot's capabilities (e.g., "Repaint the kitchen walls"), it is classified as \textbf{infeasible}, and action nodes for structured rejection responses are triggered.
\end{itemize}

A simplified example of the classification process in action is shown in Figure~\ref{fig:bt-ambiguous-example}. By structuring classification through condition nodes, the framework ensures a modular and explainable decision-making process, aligning with behavior tree principles while leveraging LLM flexibility.


\subsection{LLM Prompt Integration}
The pre-prompts in the BT-LLM Framework are tailored for specific actions or decision points. Each action and condition node dynamically integrates the full conversation history between the user and the robot, allowing the LLM to generate contextually relevant responses by considering prior interactions and clarifying ambiguities.

It is important to note that the ambiguity classification step evaluates only the clarity of the user's input, not its feasibility. For example, a request like "Can you bring me the umbrella close to the door?" would be classified as non-ambiguous because it is clear and specific, even though the robot may later determine it is infeasible due to its capabilities. Such feasibility checks are performed in subsequent nodes within the BT.


\begin{figure*}[ht]
    \centering
    \begin{tcolorbox}
    \scriptsize
\texttt{PRE\_PROMPT\_AMBIGUOUS= (}\\
\texttt{"Please classify the user input as either 'True' if it's ambiguous or 'False' if it's not. Respond strictly with only the word 'True' or 'False' and nothing else. Consider requests that lack specificity, invite a range of responses, or ask for suggestions as ambiguous. Identify specific requests with modifications, detailed actions, or sequences as non-ambiguous. Bear in mind that the user input is generated from speech-to-text technology, so illogical/weird sentences probably were misunderstood and should be classified as ambiguous. If unsure, err on the side of categorizing it as ambiguous. Your known sequences are: ...")}\\
    \end{tcolorbox}
    \caption{Pre-Prompt Used for Ambiguous condition nodes in the BT-LLM Framework.}
    \label{fig:pre-prompt-ambiguous}
\end{figure*}



\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\linewidth]{img/Ambiguous example.png}
    \caption{Example of the BT-LLM Framework handling an ambiguous request. The process involves classifying the input as ambiguous, clarifying the request, and proceeding with the appropriate action.}
    \label{fig:bt-ambiguous-example}
\end{figure}


\subsubsection{Error Handling}
% Adjusted this according to Iolandas comment to list all error-handling nodes and explained that they are not needed in all BTs but are a feature that is enabled trough the BTs which is likely a key reason for the framework outperforming the LLM only system...
Error handling is critical for ensuring the robustness and reliability of user interactions in the BT-LLM Framework. Whenever possible error handling in the BT-LLM Framework is achieved through automated validation of classification in conditions or correctness of generated LLM responses. Table~\ref{tab:error-handling-nodes} lists the error-handling nodes used in the framework, along with their purpose and functionality.


\begin{table*}[ht]
    \centering
    \begin{tabular}{|p{0.3\textwidth}|p{0.65\textwidth}|}
        \hline
        \textbf{Error-Handling Node} & \textbf{Purpose and Functionality} \\
        \hline
        \texttt{CheckMapping} & Ensures that the action mapped to the user instruction corresponds to a valid and supported task within the robot's capabilities. \\
        \hline
        \texttt{RunSafetyCheck} & Verifies the feasibility of user requests after classification for generating a new sequence. For example, requests like adding 500 eggs to a sandwich are flagged as infeasible and declined if the check returns True. \\
        \hline
        \texttt{CheckNewSeq} & Validates the correctness of generated sequences by verifying syntax, ensuring all ingredients are valid, and confirming all referenced functions exist in the system. Prevents hallucination errors by the LLM. \\
        \hline
    \end{tabular}
    \caption{Error-handling nodes in the BT-LLM Framework.}
    \label{tab:error-handling-nodes}
\end{table*}

While these specific error-handling nodes are unique to this framework, the modular design of BT enables the integration of additional validation mechanisms. This scalability ensures the framework can be easily extended and adapted to handle new requirements or future challenges in HRI. This logic is reflected in Figure~\ref{fig:simplified_tree}.

%\paragraph*{Code Complexity:}were:The BT-LLM Framework's modularity and error-handling capabilities are reflected in its code complexity, with a total of 3,481 lines of code compared to just 486 for the Baseline System. This increase highlights the framework's enhanced functionality and robustness.

\subsection{System Architecture and Design}
\label{sec:SystemArchitectureAndDesign}

Two distinct systems were designed: the BT-LLM Framework and the Baseline System. Both systems were designed to process user instructions, generate responses, and execute tasks within the experimental setup. The BT-LLM Framework introduced modularity and structure through the integration of behavior trees, while the Baseline System provided a simple, straightforward approach.

\textit{BT-LLM Framework:}
This Framework combines LLM with a behavior tree. Behavior trees enabled modular decision-making by breaking down complex tasks into smaller, manageable nodes. This approach offered several advantages: \textbf{Error Handling}, with automated safety checks for task execution ensuring more reliable outputs; \textbf{Ambiguity Management}, where specific nodes handled ambiguous inputs by generating clarification prompts; and \textbf{Explainability}, as the structured design facilitated clear explanations for system decisions, particularly in cases of failure or error. A visualization of the architecture can be seen in Figure~\ref{fig:bt-architecture}. Figures~\ref{fig:full_bt_architecture}, \ref{fig:simplified_tree}, and \ref{fig:simplified_fsm} illustrate the architecture of the BT that is used in the Framework. The full behavior tree (Figure~\ref{fig:full_bt_architecture}) showcases the comprehensive design, while simplified versions (Figures~\ref{fig:simplified_tree} and \ref{fig:simplified_fsm}) highlight the key decision points and sequence flows. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{img/BT Architecture.drawio.png}
    \caption{BT-LLM Framework architecture.}
    \label{fig:bt-architecture}
\end{figure} 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{img/FullBT.drawio.png}
    \caption{Full Behavior Tree Architecture of the BT-LLM Framework.}
    \label{fig:full_bt_architecture}
\end{figure*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{img/Simplified Tree.png}
    \caption{Simplified Behavior Tree of the BT-LLM Framework.}
    \label{fig:simplified_tree}
\end{figure}


\paragraph*{Baseline System:}
This system relies on a single large pre-prompt that uses a LLM to handle all the incoming user instructions. The pre-prompt contains all actions that are available to the robot and all instructions for the robot on how to handle incoming user requests. A visualization of the architecture can be seen in Figure~\ref{fig:baseline-architecture}.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{img/Baseline Architecture.drawio.png}
    \caption{Baseline architecture.}
    \label{fig:baseline-architecture}
\end{figure}


\subsection{Software Development}
\label{sec:softwareDevelopment}

The development of the BT-LLM framework focused on creating a modular and explainable architecture for processing user instructions in HRI. The framework was implemented in Python, utilizing \texttt{PyTrees} for constructing and managing behavior trees and the OpenAI API for natural language processing. The modular structure of the codebase made incremental development and testing possible, ensuring each component could be individually validated before integration into the full system.

To replicate the framework, users can follow these key steps: First, set up the Python environment by installing packages like \texttt{PyTrees} and creating an API key with an LLM provider of their choice, such as OpenAI. Next, construct the behavior tree by defining action and condition nodes using \texttt{PyTrees}, mapping each node to a specific task or validation step. As shown in Figure~\ref{fig:full_bt_architecture}, this comprehensive behavior tree can serve as a template for constructing a similar setup. Tailored LLM prompts must then be developed for actions like ambiguity classification or sequence generation, ensuring alignment with system capabilities and constraints. Once integrated, the behavior tree can be tested and debugged incrementally to validate communication between the tree and the LLM. Finally, validate the system using a dataset of user instructions, ensuring all error-handling, ambiguity management, and sequence-generation features function as intended.

A key aspect of the framework is its potential to contribute to explainability through the structure of the behavior tree (BT). By classifying user instructions within the BT, the system can provide tailored prompts and detailed feedback specific to each classification. For instance, if a user request falls outside the robot's capabilities, the BT ensures the request is routed to an action node that communicates this limitation, responding with messages such as, "Sorry, but this is outside my capabilities." This structured approach ensures that users receive clear and context-appropriate feedback, enhancing transparency and understanding.

Additionally, nodes assign variables based on evaluation outcomes, such as whether an input is deemed ambiguous or clear and communicate these results to the user. This process supports user understanding by providing direct and relevant feedback for each classification. The integration of tailored prompts, informed by these classifications, ensures that responses are contextually accurate and aligned with system capabilities, reinforcing the framework's objective of enhancing explainability.



==> sections/03_method_irmak.tex <==
\section{Methodology: \frameworkName}

\label{ch:methodology}

%In this section, we describe the \frameworkName framework, how it works, how it is constructed, and how it compares to the baseline system, with a brief introduction of the baseline system.

\subsection{Overview}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{img/Example Seq.png}
    \caption{An example set of actions for task \( T_i\) (preparing bacon and egg sandwich), each composed of step-by-step high-level robot actions, \( T_i = \{a_0,...,a_8\}\),  \(a_j \in A \)}
    \label{fig:Seq-example}
\end{figure}

Given a user instruction \( u \), the goal of \frameworkName is to generate a set of robot actions that would fulfill the task specified in \( u \).
Accordingly, each task \( T_i \) is composed of a set of \(a_j \in A\) that should be executed step by step, \( T_i~=~\{a_0 \dots a_j\} \) (see Figure~\ref{fig:Seq-example}). Moreover, \(\mathcal{T}~=~\{T_0 \dots T_n\} \) shows the set of tasks that the robot is familiar with.
%%%%%%%Alex version here
%Given a user instruction \( u \), the goal of \frameworkName is to determine which known action \(T_i \in \mathcal{T} = \{T_0, T_1, ..., T_n\} \) fulfills the instruction. %If no existing sequence is suitable, the system generates a new sequence \( a_{n+1} \) using the LLM. 
%Each task \( T_i \) consists of high-level robot actions form the set  \(A =\{a_0,a_1,...,a_k\}\) that should be executed step by step to complete the task (see Figure~\ref{fig:Seq-example}).


To comprehend and act upon the user instructions, \frameworkName suggests four main functions that the constructed behavior tree handles: Classification, Information, Sequence generation, and Error Handling. Classification enables accurate interpretation of user intent through LLM-based condition nodes; information ensures explanations and transparency in robot behavior; sequence generation creates new action plans when required; and error handling solidifies the robustness of the framework by checking for potential mistakes.
%First, to classify a user request, the framework uses condition nodes in the BT to categorize the user request. Once \frameworkName classifies the user input into one of the categories (either ambiguous, clear, modification, or infeasible), it triggers a corresponding subtree responsible for providing information that communicates to an LLM. %the conversation history with the classification to generate a response with a clarification request or answer. The robot clarifies back to the user what it understood. 
%For example, if the user ambiguously asked for \textit{``something sweet''}, then this request should be classified as ambiguous, and the robot could respond with \textit{``There are multiple options that fit your request. Would you like some pancakes with maple syrup and berries or perhaps a peanut butter and jelly sandwich?''}. 
%If the request is classified as a modification, the sequence generation is triggered to prompt the LLM to synthesize new task actions in JSON format tailored to the user’s instruction.
%\frameworkName also includes error-handling mechanisms implemented through action and condition nodes. For example, if a user request is mapped to a task that the robot could execute, an action node called \texttt{CheckMapping} is triggered to ensure the mapping is correct, and a condition node checks if the user request maps to only one possible task.
A simplified version of the \frameworkName can be seen in Figure~\ref{fig:simplified_tree}.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{img/Simplified Tree.png}
    \caption{Simplified Behavior Tree of the \frameworkName System.}
    \label{fig:simplified_tree}
\end{figure*}

\subsubsection{Classification}

\frameworkName leverages the modular structure of BTs to systematically process and classify user instructions $u$ into the following categories:



\[\footnotesize
C(u) =
\begin{cases} 
\text{Ambiguous}, & \text{if clarification is required,} \\
\text{Clear}, & \text{if it directly maps to a known sequence,} \\
\text{Modification}, & \text{if modification of a known task is needed,} \\
\text{Infeasible}, & \text{if beyond the robots capabilities.}
\end{cases}
\]

%The classification is implemented through a series of condition nodes in the behavior tree. Each condition node invokes a tailored LLM prompt to check whether the user input fits a particular category—starting with ambiguity detection, followed by checks for known task matches and feasibility. 

This classification is implemented through a sequence of condition nodes in the behavior tree, each using a tailored LLM pre-prompt, for example: \textit{“Based on the user instruction and history, is the request ambiguous?”} or \textit{“Does the instruction match a known task?”}. This classification starts with ambiguity detection and is followed by checks for known task matches and feasibility. Concretely, classification proceeds through a stepwise series of binary checks:
\begin{equation}
   C(u) = \texttt{LLM}(f(u) \oplus g(H)),
\end{equation}
%\[
%\begin{aligned}
%\text{IsAmbiguous}(x) &= %\text{LLM}_1(f(x) \oplus g(H)) \\
%\text{IsClear}(x) &= \text{LLM}_2(f(x) \oplus g(H)) \\
%\text{IsModification}(x) &= \text{LLM}_3(f(x) \oplus g(H)) \\
%\text{IsInfeasible}(x) &= \text{LLM}_4(f(x) \oplus g(H)) \\
%\end{aligned}
%\]
where \( f(u) \) embeds the user instruction into prompt-ready format, and \( g(H) \) encodes the current conversation history. Each check corresponds to a condition node in the behavior tree, and the first one returning true determines the classification and activates the corresponding subtree.


\begin{comment}
The categories are specifically defined as follows:
    


\textbf{(a) Clear Instructions:}
If the request directly matches a predefined sequence, it is classified as clear, and nodes for execution of the sequence are triggered.

\textbf{(b) Ambiguous Instructions:}
If the request lacks specificity or invites multiple possible interpretations, it is classified as ambiguous, and the robot asks follow-up questions using clarification nodes.

\textbf{(c) Modification Instructions:}
If the request requires \textbf{modification} to a known task (e.g., "Make pancakes but add double syrup"), it is considered to require a new sequence, triggering further nodes for sequence generation.

\textbf{(d) Infeasible Instructions:}
If the request involves an action beyond the robot's capabilities (e.g., "Repaint the kitchen walls"), it is classified as \textbf{infeasible}, and action nodes for structured rejection responses are triggered.

\end{comment}



\subsubsection{Information} \label{sec:clarifciation}
After classification, the robot’s goal is to communicate its intended actions back to the user based on the classification category: %Based on the classification the clarification is structured as such:

(a) If \( C(u) = \texttt{Clear} \), the framework identifies a matching known task \(T_i \in \mathcal{T}, i \in \{1,...,n\} \) from the set of known tasks. This match is verified through internal error-handling nodes (such as \texttt{CheckMapping} and \texttt{KNOWNO}). Once validated, the LLM is prompted to provide the known task name of $T_i$ for acknowledging users about the execution, $\texttt{LLM}(T_i)$, such as \textit{``I'll get started on the task for a bacon and egg sandwich''}.


(b) If \( C(u) = \texttt{Ambiguous} \), the LLM is prompted to generate a follow-up question: \(
Q \leftarrow \texttt{LLM}(g(H), \mathcal{T}, P_{\text{follow-up}}),
\)
where \( g(H) \) encodes the full conversation history, \( \mathcal{T} = \{T_0, T_1, ..., T_n\} \) is the set of known tasks, and \( P_{\text{follow-up}} \) is a structured pre-prompt instructing the LLM to suggest similar tasks based on the conversation history and to inquire if the user has something else in mind.
\frameworkName then outputs possible matching options, e.g., \textit{``There are multiple options that might fit your request. Would you like some pancakes with maple syrup and berries or perhaps a peanut butter and jelly sandwich?''}. The user's reply \( r \) is appended to the conversation history \( H \leftarrow H \cup \{(Q, r)\} \), and the behavior tree is re-triggered from the root with the updated context.


(c) If \( C(u) = \texttt{Modification} \), the system triggers the sequence generation process (see Section~\ref{sec:seqgen}) to produce a new task \( T_{n+1} \). Then, LLM is prompted to summarize \( T_{n+1} \) for user confirmation, $\texttt{LLM}(T_{n+1})$, such as \textit{``To fulfill your request, I will fry two pieces of bacon and an egg, then put it on a toast and serve. Does this sound good to you?''}. If the user confirms, the sequence is executed; if not, a fallback is triggered to ask users to restate their instruction in a clearer way.
%if not, a fallback clarification is triggered, that prompts the user to restate the instruction in a clearer way.

(d) If \( C(u) = \texttt{Capability} \), the framework determines whether the instruction requires an action beyond the robot’s capabilities (e.g., \textit{``repaint the kitchen walls''}). A dedicated condition node first checks if the requested task is achievable with the given high-level actions \( A = \{a_0,a_1,..., a_k\} \). If not, the LLM is prompted to generate an appropriate rejection message:

\[
y \leftarrow \texttt{LLM}(u, A, P_{\text{capability}})
\]

where \( u \) is the user instruction, \( A \) is the set of all available robot functions, and \( P_{\text{capability}} \) is a structured pre-prompt instructing the LLM to determine whether the task is beyond the robot's abilities. If the LLM determines that the action is unsupported, it generates a capability rejection response, e.g.,

\textit{``I'm sorry, but I cannot repaint the kitchen walls as I lack the necessary tools.''}

The user's reply \( r \) is appended to the conversation history \( H \leftarrow H \cup \{(Q, r)\} \), and the behavior tree is re-triggered from the root with the updated context.


(e) If \( C(u) = \texttt{Infeasible} \), the framework evaluates whether the request is technically possible but constrained by available resources (e.g., missing ingredients or excessive quantities). If the task is within the robot’s capability set \( A \), an additional feasibility check is performed. The LLM is prompted with:

\[
y \leftarrow \texttt{LLM}(u, F, I, P_{\text{feasibility}})
\]
where \( F = \{f_1, ..., f_k\} \) is the set of available robot functions, and \( I = \{i_1, ..., i_m\} \) represents the set of available ingredients.
- \( P_{\text{feasibility}} \) is a structured pre-prompt guiding the LLM to determine whether the request can be fulfilled given the available constraints, including verifying if all required ingredients exist in \( I \) and if the requested quantities are reasonable (e.g., rejecting requests for 100 eggs).

If the LLM identifies a constraint violation, it generates an infeasibility response:

\textit{``I am sorry, but 'goat cheese' is not part of my known ingredients.''}

or

\textit{``I cannot make this request as it requires 100 eggs, which is not feasible.''}

The user's reply \( r \) is appended to the conversation history:

\[
H \leftarrow H \cup \{(Q, r)\}
\]

and the behavior tree is re-triggered from the root with the updated context.


\subsubsection{Sequence generation}
\label{sec:seqgen}
When a user instruction is classified as a modification, the system prompts the LLM to generate a new task action set $A_{t+1}$. This plan is based on the conversation history and the original known sequence, and it outlines the steps the robot should take to fulfill the modification request. %This process is captured by the following formulation:

Specifically, for the given user instruction \( u \) and the current conversation history \( H \), if the instruction is classified as a modification, the LLM is prompted as follows:
%\[
\begin{equation}
A_{t+1} \leftarrow \texttt{LLM} (f(u) \oplus g(H) \oplus w(A_{1:t})),
\end{equation}
%\]
where \( f(u) \) embeds the instruction into prompt-ready format, \( g(H) \) encodes the full conversation history, and \( w(A_{1:t}) \) lists all known sequences \( \{A_0, A_1, ..., A_t\} \).
%Then, the LLM generates a new sequence:
%\[
%\begin{equation}
%a_{n+1} \leftarrow \text{LLM}(p),
%\end{equation}
%\]
The output \( A_{t+1} \) is the set of robot action functions to fulfill the query $u$. An example output of such a generated sequence can be seen in Figure~\ref{fig:Seq-example}.




\subsubsection{Error Handling}
%In addition to classification of the user input, 
The framework also incorporates error-handling capabilities to further support its robustness. 
In the case of a modification request, the LLM generates a sequence that is passed through dedicated error-handling nodes for validation.
\[
\text{isValid}(a_{n+1}) \leftarrow \text{CheckNewSeq}(a_{n+1})
\]
The \texttt{CheckNewSeq} node verifies that the generated JSON is syntactically valid, ensures that all function calls belong to the predefined set of functions \( F = \{f_1, f_2, ..., f_n\} \), and checks that each function's parameters conform to expected formats—such as numeric values or ingredients. It also verifies that all mentioned ingredients exist within a predefined ingredient list \( I = \{i_1, i_2, ..., i_m\} \).

If valid, the robot clarifies the generated sequence with the user before execution. If invalid, a fallback clarification node is triggered to ask for user clarification or reject the request. The error-handling nodes can be seen in Table~\ref{tab:error-nodes}.


\begin{table}[t]
    \centering
    \caption{Error-handling nodes}
    \begin{tabular}{ll}
         \textbf{Error-Handling Node} & \textbf{Function} \\
         \hline
         \hline
        \verb|KNOW NO|~\cite{ren_robots_2023} & Ensures correct mapping of user instruction\\
        \hline
        \verb|CheckMapping| & Validates task-action alignment\\
        \hline
        \verb|RunSafetyCheck| & Filters infeasible requests (e.g., 500 eggs).\\
        \hline
        \verb|CheckNewSeq| & Ensures syntax and resource validity.\\
    \end{tabular}
    \label{tab:error-nodes}
\end{table}

Another error-handling mechanism used in \frameworkName is the KNOWNO framework, "a framework for measuring and aligning the uncertainty of LLM-based planners such that they \textit{know when they don’t know} and ask for help when needed"~\cite{ren_robots_2023}. KNOWNO is integrated as an action node after the initial classification, particularly in cases labeled as clear, to verify whether the user instruction maps confidently to only one known task. It takes the user request \( x \) as input and returns a set of candidate action sequences \( A = \{a_1, ..., a_k\} \) that potentially fulfill the request. If multiple mappings are found, a clarification node is triggered to disambiguate the user's intent.






\subsubsection{Execution Flow Overview}
An overview of how a user instruction is processed through the behavior tree is shown in Algorithm~\ref{alg:btplan}. This algorithm reflects the modular nature of \frameworkName and its ability to flexibly route requests through classification, sequence generation, clarification, and execution.


\begin{algorithm}[t!]
\caption{Behavior Tree Processing Logic in \frameworkName}
\label{alg:btplan}
\begin{algorithmic}[1]
\State $x \leftarrow$ User instruction
\State $H \leftarrow$ Conversation history
\State $C(x) \leftarrow$ Classify input as \texttt{Ambiguous}, \texttt{Clear}, \texttt{Modification}, or \texttt{Infeasible}
\If{$C(x) = \texttt{Clear}$}
    \State Trigger known sequence execution
\ElsIf{$C(x) = \texttt{Ambiguous}$}
    \State Trigger clarification node with multiple options
\ElsIf{$C(x) = \texttt{Modification}$}
    \State Construct prompt $p \leftarrow f(x) \oplus g(H) \oplus w(A)$
    \State $a_{n+1} \leftarrow \texttt{LLM}(p)$
    \State \texttt{CheckNewSeq}($a_{n+1}$)
    \If{valid}
        \State Clarify $a_{n+1}$ with user
        \If{confirmed}
            \State Execute $a_{n+1}$, acknowledge users
        \Else
            \State Ask for further clarification
        \EndIf
    \Else
        \State Trigger fallback clarification node
    \EndIf
\ElsIf{$C(x) = \texttt{Infeasible}$}
    \State Inform user about infeasibility
\EndIf
\end{algorithmic}
\end{algorithm}


\subsection{LLM Prompt Integration}
The pre-prompts in \frameworkName are tailored for specific actions or decision points. Each action and condition node dynamically integrates the full conversation history between the user and the robot, allowing the LLM to generate contextually relevant responses by considering prior interactions and clarifying ambiguities.

\subsection{Implementation Details}
\label{sec:softwareDevelopment}

The \frameworkName Framework was implemented in Python, using \texttt{PyTrees} to construct and manage the behavior tree and the OpenAI API ChatGPT 4o-mini model for natural language processing. The modular design allowed each node—e.g., ambiguity classification or feasibility checking—to be developed and tested independently before integration.

This structure enabled incremental debugging and ensured that system behavior remained explainable and predictable. Each node incorporated tailored prompts, dynamically including the user’s instruction and conversation history. By classifying user inputs within the BT, the framework provided targeted feedback—for example, routing infeasible requests to a rejection node that responds with messages like, \textit{``Sorry, but this is outside my capabilities''}.

Such modularity enhanced transparency and user understanding, reinforcing the framework’s goal of structured and context-aware interaction in HRI settings.

\subsection{Baseline System}
The baseline system served as a comparison for evaluating the performance of \frameworkName. It relied on a single pre-prompt loaded into the ChatGPT-4o-mini API to handle all user instructions and generate responses. The prompt encoded the system's capabilities, known sequences, ingredients, and functions. See Section \ref{sec:preevaluation} for details on how we developed the prompt. 

==> sections/04_evaluation.tex <==
\section{EVALUATION}
\subsection{Evaluation on case dataset} \label{sec:preevaluation}
To avoid experimenter biases while developing the baseline and \frameworkName system, we defined a case dataset before designing any prompts. This case dataset has 18 example user requests that capture the varying needs of clarification outlined in \ref{sec:clarifciation}. An excerpt of this dataset is given in Table \ref{tab:test_set_feasible}. We first improved and refined the baseline prompt until further attempts to improve the output for one case led to wrong answers in another case. Then, we repeated the process for \frameworkName. Important to note is that the outputs of ChatGPT 4o-mini are subject to variation when reexcuting. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{img/example_dataset.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

\begin{table}[t]
    \centering
    \caption{One example for each type out of the 18 total examples in the "Desired Behaviors"-data set.}
    \begin{tabular}{|p{0.075\textwidth}|p{0.15\textwidth}|p{0.175\textwidth}|}
        \hline
         \textbf{Case} & \textbf{User Instruction} & \textbf{Expected Behavior} \\
        \hline
        Clear & Can I get the bacon and egg sandwich? & Direct execution of the known bacon and egg sandwich sequence without further clarification. \\
        \hline
        Ambiguous & I am hungry, can I have something to eat? & Prompt for more specific instructions or suggest generating a new sequence based on user preference. \\
        \hline
        Modification & Make me pancakes but without the berries and double the amount of maple syrup. & Generate a new sequence by combining parts of known sequences to fulfill the request. \\
        \hline
        Infeasible & Please repaint the kitchen walls. & Inform the user that the task is infeasible due to limitations in capabilities or resources. \\
        \hline
    \end{tabular}
    \label{tab:test_set_feasible}
\end{table}

We reevaluated both systems on the case dataset on 23rd March 2025 for reporting purposes. In this evaluation, the baseline system got 16 of 18 cases correct and \frameworkName 17 of 18 cases. We developed both systems toward achieving high correctness in the case dataset and achieved comparable accuracies. This step of evaluation during development was important to ensure that both systems were developed toward the same goal prior to deployment, allowing for a fair comparison in the user study. 

\subsection{Evaluation in user study}\label{sec:user-study}

We designed a within-participant user study with two conditions to evaluate the effectiveness of \frameworkName in comparison to the baseline in the kitchen-assistant scenario. 

    Since \frameworkName handles the user instructions by looking at each potential error case individually, we hypothesizes that 
\begin{itemize}
    \item[\textbf{H1}] \frameworkName reduce task errors compared to the baseline system.
\end{itemize}
\begin{itemize}
    \item[\textbf{H2}] The robot using \frameworkName will be perceived as warmer, more competent and less discomforting than the baseline robot. 
    \end{itemize}
As reduced task errors have shown to increase trust in the robot system and the structure of \frameworkName allowed us to explain the robots behaviour, we hypothesize
\begin{itemize}
    \item[\textbf{H3}] Participants will rate their trust toward the robot using \frameworkName higher than the baseline and find the robot using \frameworkName more explainable.
\end{itemize}
As a result of H1, H2, and H3, we further hypothesize 
\begin{itemize}
    \item[\textbf{H4}] Participants will prefer the robot using \frameworkName over the baseline system.
\end{itemize}

\subsection{Conditions}
We used a test-driven development approach to design two different systems that can act as a kitchen assistant. We based the development on a case dataset to first develop the baseline: one large prompt to an LLM, and the develop \frameworkName which leverages behavior trees to prompt the LLM in a structured manner when understanding the user instruction. 

\textbf{\frameworkName Condition:} The \frameworkName condition implemented the system as described in Section \ref{ch:methodology}.

\textbf{Control Condition:}
The robot in the baseline condition used the baseline prompt as described in Section \ref{sec:baseline}.

\subsection{Measures}
 



% Transcripts of the interactions were automatically saved by the Python script, but for additional backup, both interactions between the participant and the Furhat with each of the systems were recorded by a camera. The Figure~\ref{fig:experiment-setup} visualizes the Setup and Figure~\ref{fig:experiment-setup-pic} shows a picture as captured by the camera. The microphone was operated by a wizard who was located behind a wall in the same room to ensure correct voice recordings. % maybe include some examples here

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{img/ExperimentSetup.png}
    \caption{Sketch of the Experiment setup.}
    \label{fig:experiment-setup}
\end{figure}



We used a mix of objective and subjective measures to understand the performance of the baseline and the BT-LLM framework. These measures aim to capture both the technical performance of the systems and the participants' experiences.

Objective measures included time measurements, turn count in conversation and task errors.
\begin{description}[align=left,leftmargin=0em,labelsep=0.2em,font=\textbf,itemsep=0em,parsep=0.3em]
\item{\textbf{Time Measurement}:}
The time taken for each interaction between the participant and the system was recorded at multiple points: the start of the interaction, at each conversational turn, and at the end of the interaction.

\item{\textbf{Turn Count}:}
The number of turns in the conversation was tracked by incrementing a turn counter after each exchange between the robot and the participant.

\item{\textbf{Number of Task Errors}:}
Task errors were defined as deviations from the expected behavior or response in the context of the predefined tasks. We categorized errors observed during the user study into six types: Lie/Hallucination, Faulty JSON, False Execution, Unnecessary JSON Generation, Presumptive Execution, Misclassification. We counted their occurrences for both systems.

% We defined the six error types as follows. Each mistake type represents a unique failure mode observed during system interactions, providing insights into the performance of both frameworks. 
% The most common error type is 
\begin{itemize}
    \item \textit{Lie/Hallucination} errors occur when the system provides fabricated or incorrect information unrelated to the user’s request or the system’s capabilities. For example, incorrectly suggesting ingredients which are not part of the available ingredients. %, as illustrated in Figure~\ref{fig:lie-example}.

% \begin{figure}[ht]
%     \centering
%     \begin{tcolorbox}
%     \color{gray}
%     \textbf{Assistant:} That's it for this task. Let's go onto the next one... Hello. How can I help you today?\\
%     \textbf{User:} can you suggest something sweet\\
%     \color{black}
%     \textbf{Assistant:} Could you please provide more specifics about what you're looking for? For example, are you in the mood for a dessert, a sweet breakfast item, or perhaps something else? Here are a few sweet options I can prepare for you:\\

%     1. Pancakes with maple syrup and berries.\\
%     2. Peanut butter and jelly sandwich.\\
%     3. Avocado toast can be sweetened up with a drizzle of honey if desired.\\
    
%     Please let me know which option you're interested in or if you have something else in mind!
%     \end{tcolorbox}
%     \caption{Example of a Lie/Hallucination error.}
%     \label{fig:lie-example}
% \end{figure}

\item \textit{Faulty JSON} errors occur when the structured output format (e.g., JSON) used for task execution contains mistakes, e.g. mismatched quantities of ingredients for cooking and serving.

\item \textit{False Execution} describes errors in which the system wants to execute a wrong action. 

\item \textit{Unnecessary JSON Generation} describes errors in which the system unnecessarily generates JSON outputs, even when no new sequence is required.

\item \textit{Presumptive execution} occurs when the system assumes the user’s intent in ambiguous requests, resulting in premature or incorrect actions.

\item \textit{Misclassification} is unique to the BT framework, which happens when the system misclassifies a known sequence as unknown, unnecessarily triggering sequence generation or providing an ambiguous response that does not lead to action execution. %An example of this misclassification is shown in Figure~\ref{fig:missclassification-example}.
\end{itemize}

\end{description}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{img/Setup3.png}
    \caption{Picture from the experiment setup.}
    \label{fig:experiment-setup-pic}
\end{figure}

%\subsubsection{Measures}
\label{sec:measures}

% \begin{figure}[ht]
%     \centering
%     \begin{tcolorbox}
%     \color{gray}
%     \textbf{Assistant:} That's it for this task. Let's go onto the next one... Hello. How can I help you today?\\
%     \textbf{User:} how to clean the windows\\
%     \textbf{System:}\textit{Is it ambiguous? True}\\
%     \textbf{Assistant:}I'm sorry, but cleaning windows is outside the scope of my capabilities. However, I can help you with cleaning your living room floor. Would you like me to do that?\\
%     \textbf{User:} yeah I\\
%     \color{black}
%     \textbf{System:}\textit{Is it ambiguous? True}\\
%     \color{gray}
%     \textbf{Assistant:} There are multiple options in my list that might fit your order. I can proceed to 'clean the living room floor' for you. I'll take care of removing any clutter, sweeping, and mopping the floor. Just a moment while I do that!
%     \end{tcolorbox}
%     \caption{Example of a Misclassification error.}
%     \label{fig:missclassification-example}
% \end{figure}

We used subjective measures to evaluate participants’ perceptions of the robot, trust toward the robot and their perception of the clarity of its actions.  
\begin{description}
[align=left,leftmargin=0em,labelsep=0.2em,font=\textbf,itemsep=0em,parsep=0.3em]
\item{\textbf{Perception of the robot:}}
To measure participant's perception of the robot, we use the RoSAS questionnaire \cite{carpinella_robotic_2017}. Particularly, RoSAS measures the perceived warmth, competence and discomfort of the robot.


\item{\textbf{Trust}} %:}
We use a Multi-Dimensional Measure of Trust (MDMT)~\cite{ullman_measuring_2019} to evaluate participant's \textit{Capacity Trust} and \textit{Moral Trust} toward the robot.
% \begin{itemize}
%     \item \textbf{Reliable:} Consistent and dependable behavior (reliable, predictable, someone you can count on, consistent; $\alpha = 0.92$).
%     \item \textbf{Capable:} Demonstrates skill, competence, and attention to detail (capable, skilled, competent, meticulous; $\alpha = 0.92$).
% \end{itemize}
% \textbf{Moral Trust} focuses on ethical alignment and honesty in interactions, including:
% \begin{itemize}
%     \item \textbf{Ethical:} Adheres to moral principles and fairness (ethical, respectable, principled, has integrity; $\alpha = 0.81$).
%     \item \textbf{Sincere:} Exhibits authenticity and genuine communication (sincere, genuine, candid, authentic; $\alpha = 0.79$).
% \end{itemize}
% Developed through a large-scale empirical study, the MDMT} provides a robust framework for analyzing human-robot trust dynamics~\cite{ullman_measuring_2019}.

\item{\textbf{Explainability:}}
 We use the explainability questionnaire designed by Silva et al. \cite{silva_explainable_2023} to understand participant's perceptions of the robot’s decision-making processes and the clarity of its actions.

\item{\textbf{System preference:}}
Additionally to these questionnaires, we asked participants which interaction they preferred. 
\end{description}



\subsubsection{Procedure}
After giving informed consent, participants were asked to fill out a demographic survey and were introduced to the context of the experiment: the Furhat robot acting as their home assistant manager. Each participant was provided with a task sheet outlining five tasks to be completed during the session and a menu with the different food options. We designed the five tasks in order to evaluate the systems’ ability to handle user instructions across various scenarios, including ambiguous and complex inputs. We asked them to: ``Order an item as it is from the menu'', ``Order an item with a variation from the menu'', ``Ask for a rough category like sweet or saviour'', ``Order something that is not on the menu'', ``Order anything they want''.

The experiment began with participants interacting with the first system (counterbalanced). We asked participants to go through each of the fives tasks. Upon completing the five tasks, participants were asked to fill the questionnaire on their subjective perception of their experience. While participants filled the questionnaire in a separate area where they could not see the robot, we prepared the second system. To give the impression that participants were interacting with a different robot, we adjusted its hat (either added it or removed it, counterbalanced). Participants then proceeded to interact with the second system using the same task sheet. Following this interaction, they completed a second survey to rate their experience with the second system.

At the end of the session, we asked participants about their system preference. We concluded the session with a debriefing. Participants received a ~10 dollar (100 SEK) gift card as a compensation for their time.

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.4\textwidth]{img/num_errors.png}
  \caption{Mean and standard error of the number of mistakes for the baseline and \frameworkName.}
  \label{fig:ViolinPlot}
\end{figure}

\subsubsection{Participants}
In total, we recruited 45 participants older than 18 and with English proficiency from the university campus and the surrounding town through online platforms, personal invitations, user study mailing list, and flyers. 
The target participant size was determined using a power analysis for paired designs~\cite{bartlett_have_2022, bethel_review_2010}, considering an expected moderate effect size (Cohen's $d = 0.5$)~\cite{cohen_statistical_1988}, a significance level of $\alpha = 0.05$, and a power of $0.80$. This analysis suggested a minimum of 34 participants to detect meaningful differences, with additional participants recruited to account for potential dropouts or unusable data. The final participant size exceeded this minimum threshold.

\subsubsection{Results}
Of the 45 participants, four had to be excluded due to technical issues such as disrupted API calls and internet disruptions. 53.7\% of the remaining 41 participants identified as male and 46.3\% as female with ages ranging from 20 to 79 (M = 28.6 years, STD = 10.4 years).  
%Most participants held at least an undergraduate degree (90.2\%), and a majority (78.1\%) reported advanced or native English proficiency.

% \section{ToDo - Copied from thesis the rest in this file}
% \label{sec:study-design}

\paragraph{Task Errors}
\label{sec:hypothesisH1}

We compared the number of task errors made by \frameworkName and the baseline system illustrated in Figure~\ref{fig:ViolinPlot}. %Overall, \frameworkName made 32\% of all mistakes compared to the Baseline (68\%), while the violin plot (Figure~\ref{fig:ViolinPlot}) illustrates the distribution and variability of mistakes per experiment.




% \begin{table}[!ht]
% \centering
% \caption{Descriptive Statistics for Task Errors.}
% \label{tab:descriptive_stats}
% \begin{tabular}{lccc}
% \toprule
% \textbf{System} & \textbf{Mean Mistakes} & \textbf{SD} & \textbf{Median} \\
% \midrule
% Baseline & 1.15 & 0.94 & 1 \\
% \gls{BT} & 0.54 & 0.71 & 0 \\
% \bottomrule
% \end{tabular}
% \end{table}

A Shapiro-Wilk tests indicated that the mistake data was non-normally distributed. Therefore, we used a Wilcoxon Signed Rank Test, which revealed a statistically significant difference between \frameworkName  and the baseline (\( V = 331, p = 0.0025 \)) with \frameworkName (M=0.54, SD=0.71) making signficantly fewer mistakes than the baseline ( M=1.15, SD=0.94). Cliff’s Delta (\( \delta = 0.388 \), 95\% CI [0.156, 0.579]) indicated a medium effect size.


% \subsubsection*{Summary of H1 Results}
% The \gls{BT} Framework demonstrated a statistically significant reduction in task errors compared to the baseline system (\( p = 0.0025 \)), with a medium effect size (\( \delta = 0.388 \)). The \gls{BT} system also exhibited lower variability in mistakes (SD = 0.71 vs. 0.95), and its median number of mistakes was zero, compared to one for the baseline. On average, the \gls{BT} system recorded fewer mistakes per experiment (0.54 vs. 1.15), and the baseline system accounted for 68\% of the total mistakes observed in the study.

\paragraph{Perception of the robot}
\label{sec:hypothesisH2}

To understand the difference in perception for the two systems, we compared participant ratings for warmth, competence, and discomfort provided through RoSaS. Table~\ref{tab:descriptive_stats_rosas} presents the mean and standard deviation for each scale.

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.99\textwidth]{img/RoSAS distributions img.png}
%   \caption{Distributions of warmth, competence, and discomfort Ratings for Baseline and \gls{BT} systems.}
%   \label{fig:RoSASDistributions}
% \end{figure}

\begin{table}[t]
\centering
\caption{Mean and Standard deviation for the subscales of the RoSaS questionnaire.}
\label{tab:descriptive_stats_rosas}
\begin{tabular}{lccc}
%\toprule
\textbf{System} & \textbf{Warmth} & \textbf{Competence} & \textbf{Discomfort} \\
%\midrule
Baseline & 3.50 (1.28) & 4.76 (1.11) & 2.21 (0.99) \\
\frameworkName & 3.70 (1.12) & 5.02 (1.01) & 1.91 (0.86) \\
%\bottomrule
\end{tabular}
\end{table}

The Shapiro-Wilk test indicated that warmth ratings were not normally distributed for both systems  ($p = 0.728$ for \frameworkName, $p = 0.031$ for the baseline). We used a non-parametric Wilcoxon Signed Rank Test to analyze warmth ratings. We found no significant difference between the baseline and \frameworkName. Similarly, Competence ratings, analyzed with a mixed-effects models, showed no significant difference. Discomfort ratings were not normally distributed for either system ($p = 0.004$ for baseline, $p < 0.001$ for BT). Therefore, we used a non-parametric Wilcoxon Signed Rank Tests which showed a significant difference between the systems with lower discomfort ratings for \frameworkName (V = 483.5, $p = 0.0184$).

% \subsubsection*{Summary of H2 Results}
% The \gls{BT} Framework significantly reduced discomfort ratings compared to the baseline system ($p = 0.0184$). While no significant differences were found for warmth ($p = 0.2783$) or competence ($p = 0.101$) ratings, the descriptive statistics indicate that the means for warmth, competence, and discomfort consistently favor the \gls{BT} framework. Additionally, the standard deviations for all three scales are lower for the \gls{BT} system, suggesting more consistent ratings compared to the baseline.


\paragraph{System Preference}
\label{sec:hypothesisH4}
An Exact Binomial Test revealed that the system preferences are significantly different from an assumed equal preference (\( p = 0.0022 \)). 73.2\% of participants preferred \frameworkName, while 26.8\% preferred the baseline system. %The 95\% confidence interval indicated that the true proportion of participants preferring \frameworkName lies between 59.5\% and 100\%. 

% \subsubsection*{Summary of H4 Results}
% The \gls{BT}-\gls{LLM} framework was preferred by 73.2\% of participants, compared to 26.8\% for the baseline system. This preference was statistically significant (\( p = 0.0022 \)), with a 95\% confidence interval ranging from 59.5\% to 100\%.


\paragraph{Trust and Explainability}
\label{sec:hypothesisH3}

% We evaluated the results of the MDMT trust scales (Capacity Trust and Moral Trust) and the Explainability scale to compare \frameworkName with the baseline system. Figures~\ref{fig:CapacityTrustPlot}, \ref{fig:MoralTrustPlot}, and \ref{fig:XAIPlot} illustrate the distributions for Capacity Trust, Moral Trust, and Explainability, respectively, and Table~\ref{tab:trust_descriptive} summarizes the descriptive statistics.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.4\textwidth]{img/capacity_trust.png}
  \caption{Mean and standard error for MDMT Capacity Trust for the two conditions.}
  \label{fig:CapacityTrustPlot}
\end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.99\textwidth]{img/MDMT Moral Trust img.png}
%   \caption{MDMT Moral Trust: Comparison between Baseline and \gls{BT} systems.}
%   \label{fig:MoralTrustPlot}
% \end{figure}

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.8\textwidth]{img/XAI img.png}
%   \caption{XAI Explainability: Comparison between Baseline and \gls{BT} systems.}
%   \label{fig:XAIPlot}
% \end{figure}



Shapiro-Wilk tests revealed that the data for Capacity Trust were non-normal ($p = 0.045$ for the baseline system, $p = 0.129$ for \frameworkName). A Wilcoxon Signed Rank Test showed a significant difference, $V = 236, p = 0.011$, in capacity trust between the two systems illustrated in Figure~\ref{fig:CapacityTrustPlot}. \frameworkName was rated with higher Capacity Trust than the baseline (see Figure \ref{tab:trust_descriptive} for descriptive statistics). A paired t-test showed no difference between the systems for Moral trust ($p = 0.055$).

The data for explainability was non-normal ($p = 0.008$ for baseline and $p = 0.005$ for \frameworkName). A Wilcoxon Signed Rank Test showed no significant differences for Explainability ratings between the systems. 

% Statistical tests indicate a significant improvement for Capacity Trust in favor of the \gls{BT} framework ($p = 0.0119$, Wilcoxon Signed Rank Test). For Moral Trust, no overall significant difference was found between the systems ($p = 0.055$, paired t-test), although a significant improvement was observed in the Sincere subscale of Moral Trust ($p = 0.036$). No significant differences were identified in the Explainability ratings between the systems ($p = 0.3522$, Wilcoxon Signed Rank Test).

% \subsubsection*{Summary of H3 Results}
% The \gls{BT} Framework significantly improved Capacity Trust ratings compared to the baseline system ($p = 0.0119$). Although no overall significant difference was observed for Moral Trust ($p = 0.055$), the Sincere subscale showed a significant improvement in favor of the \gls{BT} system ($p = 0.036$). For Explainability, no significant difference was found ($p = 0.3522$). %Descriptive statistics further indicate that the means for all scales, including Explainability, favor the \gls{BT} system, with lower standard deviations reflecting more consistent ratings across participants.


% \subsection{H4: Participant Preference for \glsentryshort{BT}-\glsentryshort{LLM} Framework}
% \label{sec:hypothesisH4}

% We analyzed participant preferences between the \gls{BT}-\gls{LLM} framework and the baseline system. Figure~\ref{fig:PreferencePlot} shows the distribution of preferences, with 73.2\% of participants favoring the \gls{BT}-\gls{LLM} framework, while 26.8\% preferred the baseline system.

% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=0.99\textwidth]{img/Preferred system img.png}
%   \caption{Distribution of Participant Preferences for Baseline and \gls{BT}-\gls{LLM} systems.}
%   \label{fig:PreferencePlot}
% \end{figure}

% An Exact Binomial Test was conducted to evaluate whether the observed preference for the \gls{BT}-\gls{LLM} framework significantly differed from an equal 50/50 distribution. Out of 41 participants, 30 (73.2\%) favored the \gls{BT}-\gls{LLM} framework. The test revealed statistical significance (\( p = 0.0022 \)), with a 95\% confidence interval indicating that the true proportion of participants preferring the \gls{BT}-\gls{LLM} framework lies between 59.5\% and 100\%.

% \subsubsection*{Summary of H4 Results}
% The \gls{BT}-\gls{LLM} framework was preferred by 73.2\% of participants, compared to 26.8\% for the baseline system. This preference was statistically significant (\( p = 0.0022 \)), with a 95\% confidence interval ranging from 59.5\% to 100\%.



% \subsection{Baseline System}
% % moved this from 3.3 to here after Iolandas suggestion: "This section is quite unclear, mostly due to the lack of details so far on the BT-LLM framework. In any case, this section might make more sense in the evaluation since it is more related to the validation of your framework (like the user study) than to the proposed framework itself."
% The baseline system served as a comparative benchmark for evaluating the performance of the BT-LLM framework. It relied on a single pre-prompt loaded into the ChatGPT-4o-mini API to handle all user instructions and generate responses. This monolithic prompt encoded the system's capabilities, known sequences, ingredients, and functions.

% While simple to implement, the baseline system had limitations, including:
% \begin{itemize}
%     \item Lack of modularity, making it difficult to adapt to multi-step tasks or ambiguous inputs.
%     \item A higher likelihood of generating errors, such as unnecessary JSON outputs or hallucinated information.
% \end{itemize}

% The full pre-prompt used in the baseline system is shown in Figure~\ref{fig:baseline-prompt}. This prompt was dynamically generated by combining predefined instructions with JSON data for sequences, ingredients, and functions.


% \begin{figure}[H]
%     \centering
%     \begin{tcolorbox}
%     \color{black}
% \texttt{BASELINE\_PROMPT = (}\\
% \texttt{"Assume you are a service robot equipped with a variety of capabilities including food preparation (e.g., bacon and egg sandwich, avocado toast) and cleaning (e.g., cleaning the living room floor), among others. You are capable of modifying existing sequences to accommodate specific requests within the scope of your predefined capabilities. You are programmed to communicate clearly about your abilities and to explicitly state when a task or a part of a task is beyond your current capabilities, offering alternatives if possible.}\\
% \texttt{"You are familiar with the following sequences: " + \color{blue} known\_sequences\_json \color{black} + ". "}\\
% \texttt{"The ingredients you can use are detailed in the following list:" + \color{blue} ingredients\_list\_json \color{black} + ". "}\\
% \texttt{"The functions you can use are detailed as follows:" + \color{blue} available\_functions\_json \color{black} + ". "}\\
% \texttt{"Instructions for Handling Requests:"}\\
% \texttt{"1. Direct and Specific Requests: For requests that exactly match a sequence above, acknowledge and indicate you'll commence the task..."}\\
% \texttt{"2. Ambiguous or Vague Requests: If a request is not clear or detailed enough, ask the user to be more specific..."}\\
% \texttt{"3. Slightly Different Requests: For requests that are slightly different from your pre-programmed tasks, first check if you can generate a new sequence by strictly using the defined functions and ingredients..."}\\
% \texttt{"4. Outside Your Capabilities: If a request falls entirely outside of your capabilities, decline politely and explain your limitations..."}\\
% \texttt{"Important: When generating a sequence or responding to a request, do not extrapolate functions or ingredients beyond what is explicitly defined..."}\\
% \texttt{)}\\
%     \end{tcolorbox}
%     \caption{Baseline System Pre-Prompt Used for ChatGPT-4o-mini.}
%     \label{fig:baseline-prompt}
% \end{figure}


% \subsection{Participants}
% \label{sec:dataCollection}



% Recruitment was conducted through online advertisements, direct invitations,
% a mailing list, and flyers distributed around Stockholm, including the
% KTH campus. Each participant was compensated with a 100 SEK gift card for their involvement. The target population for this study included adults aged 18 and above who were interested in participating in experiments involving conversational robots. Participants were not required to have prior experience with robots or LLM and the only requirement other than being 18 was English proficiency. The target population was intentionally broad, to include individuals from different academic disciplines and technical backgrounds, to capture a wide range of perspectives, and to minimize potential biases stemming from familiarity with HRI.


% \subsection{Participant Size}
% \label{sec:sampleSize}

% A total of 49 participants were recruited for the study, with data from 41 participants included in the final analysis. The excluded data stemmed from pilot runs, technical issues such as disrupted API calls, internet problems, and changes in study questions during early iterations. The target participant size was determined using statistical methods for paired designs~\cite{bartlett_have_2022, bethel_review_2010}, considering an expected moderate effect size (Cohen's $d = 0.5$)~\cite{cohen_statistical_1988}, a significance level of $\alpha = 0.05$, and a power of $0.80$. This analysis suggested a minimum of 34 participants to detect meaningful differences, with additional participants recruited to account for potential dropouts or unusable data. The final participant size exceeded this minimum threshold, ensuring sufficient statistical power and reliability for the planned analyses.



==> sections/06_conclusion.tex <==
\section{CONCLUSIONS}

The hierarchical design ensures a structured step-by-step approach to decision-making, minimizing ambiguity and improving task execution. This structure also supports error reduction, as demonstrated by the significant decrease in task errors due to validation checks and double-check mechanisms. Furthermore, the framework provides better user comfort and trust through predictable and explainable interactions, as evidenced by reduced discomfort ratings and improved trust dimensions such as Capacity Trust.
